Llumnix: Dynamic Scheduling for Large Language Model Serving

Inference serving for large language models (LLMs) is the key to unleashing their potential in people's daily lives. However, efficient LLM serving remains challenging today because the requests are inherently heterogeneous and unpredictable in terms of resource and latency requirements, as a result of the diverse applications and the dynamic execution nature of LLMs. Existing systems are fundamentally limited in handling these characteristics and cause problems such as severe queuing delays, poor tail latencies, and SLO violations. We introduce Llumnix, an LLM serving system that reacts to such heterogeneous and unpredictable requests by runtime rescheduling across multiple model instances. Similar to context switching across CPU cores in modern operating systems, Llumnix reschedules requests to improve load balancing and isolation, mitigate resource fragmentation, and differentiate request priorities and SLOs. Llumnix implements the rescheduling with an efficient and scalable live migration mechanism for requests and their in-memory states, and exploits it in a dynamic scheduling policy that unifies the multiple rescheduling scenarios elegantly. Our evaluations show that Llumnix improves tail latencies by an order of magnitude, accelerates high-priority requests by up to 1.5x, and delivers up to 36% cost savings while achieving similar tail latencies, compared against state-of-the-art LLM serving systems. Llumnix is publicly available at https://github.com/AlibabaPAI/llumnix.

==> discuss.tex <==
\section{\revise{Discussion}}

\paragraph{Global scheduling and local scheduling.}
\sysname{} targets global request scheduling across multiple model instances, which is complementary to local scheduling inside inference engines for each instance. In general, \sysname{}'s basic assumption about local scheduling is continuous batching~\cite{orca2022} with dynamic memory allocation~\cite{vllm2023}, which we believe will be the de facto standard due to the great advantages in throughput and cost efficiency of batching.
This is also why \sysname{} currently adopts vLLM~\cite{vllm2023}, a representative in this category, as the underline inference engine.
We also notice recent local scheduling techniques such as preemptive scheduling~\cite{wu2023fast} and fair scheduling~\cite{sheng2023fairness}.
We plan to continue to explore the interplay between the global scheduling of \sysname{} with these local scheduling techniques in future work.

\paragraph{Scheduling across model types.}
Beyond multiple model instances, LLM services can also involve multiple model \emph{types}.
Despite the universality of LLMs, people can also build model variants to adapt them to different application scenarios. 
A typical example is fine-tuning a base LLM to gain better performance (accuracy) on a specific task (\eg, coding~\cite{codellama,qwen,deepseek-coder}).
Another example is using different sizes or precisions of the base LLM to trade accuracy for throughput/latency~\cite{touvron2023llama,touvron2023llama2}. Using model variants represents an algorithmic approach to addressing the request heterogeneity of LLMs, which is orthogonal to \sysname{}'s scheduling approach. It is also possible and interesting to extend \sysname{} to scheduling across multiple model types, considering the larger tradeoff space of latency/throughput and accuracy.

% Another way to deal with request heterogeneity.
% Orthogonal and complementary. An interesting future work to explore (re)scheduling across multiple model types.

% \paragraph{Interfaces for request priorities/SLOs.}
% There are currently no explicit interfaces for setting requests priorities or SLOs in products like ChatGPT. We also have no evidence of LLM-based applications having such abstractions. However, we believe that ...

==> intro_old.tex <==

\section{Introduction (archived)}
Large language models (LLMs) such as the GPT series have achieved an unprecedented level of generation capabilities, being adopted by applications like chatbots, search engines, and content generation for various domains.
Inference serving of LLMs is a key factor determining the efficiency and user experiences of such online services.
% LLM serving typically involves a \emph{request scheduler} and an \emph{inference engine}: each request is first scheduled to one of the multiple instances of the LLM and then executed by the engine.
The system not only requires high throughput to reduce the costs for the providers, but needs to deliver low and stable latencies to meet the service-level objectives (SLOs) for end users as well.

LLM serving involves an \emph{inference engine} and a \emph{scheduler}.
Online services are typically backed by multiple instances of the LLM, where the engine runs the inference computation for each instance, and the scheduler dispatches requests and controls the scaling of the instances.
The common practice is to use an inference engine tailored for LLMs~\cite{faster2023,orca2022,vllm2023} due to their LLM-specific performance optimizations; nevertheless, people are still using generic schedulers that treat LLM inference requests just like those for a traditional DNN model.

A unique characteristic of LLM serving that distinguishes it from traditional DNNs is the \emph{autoregressive} execution: serving a request needs to run the model for multiple iterations, each deriving a single output token,
% from the original input and all previous output tokens, 
until an ``end-of-sequence'' token is generated.
% As each token participates in the generation of all following tokens, 
During this procedure, the inference engine typically caches intermediate results for each token,
% (key and value tensors used in the attention operation), 
known as the \emph{KV cache}, in GPU memory as these results will be involved in the generation of all following tokens.
With recent LLMs racing to support longer input/output sequences for broader application, the growing KV cache sizes make the GPU memory a bottleneck resource. 
% Support for longer sequences is necessary for broader application of LLMs; for example, to write a fiction (long output) or summarize a fiction (long input).
% LLMs released in 2023 have scaled to sequence lengths of 32k or even 100k, which translate to a memory consumption of ...
% Therefore, memory management for KV cache has become one of the biggest concerns in LLM serving.

The autoregressive execution determines that the resource demands of LLM serving are inherently \emph{dynamic and unpredictable}:
% which makes existing serving schedulers fundamentally fall short.
the KV cache of a request dynamically grows, and the final memory demand is not known a priori.
Existing serving schedulers, designed for traditional DNNs, instead assume that the execution is one-shot and the resource usage is deterministic.
Such a conflict makes existing systems fundamentally fall short of scheduling LLM serving efficiently.

First, given the unpredictable memory demands, the scheduler can hardly guarantee resource and performance isolation for requests. Although the scheduler can dispatch a request to an instance with enough memory at the arrival, the instance can still run out of space afterwards as the sequences of running requests become longer. In this case, certain requests have to be preempted and rescheduled,
which not only wastes compute cycles, but also leads to highly unstable latencies and SLO violations, significantly sacrificing user experiences.

% A key challenge with the memory management for LLM serving is the \emph{unpredictability} of the autoregressive generation, \ie, the final sequence lengths and KV cache sizes are not known a priori.
% % This challenge has deep implications at both the inference engine and the request scheduling levels.
% One simple approach for the inference engine
% to deal with such unpredictability 
% is to pre-allocate memory with the maximum length for each request~\cite{orca2022,faster2023}. Such over-allocation limits the serving batch size, resulting in low memory utilization and throughput.
% Therefore, the state of the art is to dynamically allocate memory as sequences grow~\cite{vllm2023}, which increases memory utilization and throughput with larger batch sizes. However, the dynamic allocation still suffers from the unpredictability because a batch can run out of memory as sequences become longer, despite enough memory in the beginning. In this case, the requests have to be preempted and rescheduled,
% which not only wastes compute cycles, but also leads to highly unstable latencies and SLO violations, significantly sacrificing user experiences.

Furthermore, the unpredictable memory demands introduce conflicting scheduling objectives and complex tradeoffs.
The request preemption problem above suggests a clear objective for loading balancing across instances to reduce preemptions of running requests.
Another important objective is to reduce queuing delays for new requests, especially those with long inputs and require large amounts of memory; this objective, on the contrary, prefers packing requests to fewer instances to leave other instances free to accommodate long inputs. 
% Consider the request preemption problem above, one clear objective is to reduce such preemptions for running requests; a good choice here would be spreading requests uniformly to avoid overloading certain instances.
% However, when considering incoming requests, 
% Another objective, however, is to reduce the queuing delays for new requests, especially those with long inputs and require large amounts of memory. Then the preferred choice might instead be packing requests to fewer instances to leave other instances free to accommodate long inputs.
Such conflicting objectives, combined with unpredictable request arrivals and sequence lengths, make it difficult to make an optimal scheduling decision at request arrival.

% Beyond the inference engine level, the memory challenge further complicates the
% request scheduling across model instances, introducing complex tradeoffs between conflicting scheduling objectives.
% Consider the aforementioned dynamic memory allocation, one clear objective is to reduce preemptions of running requests;
% then the system would prefer to spread requests uniformly to avoid overloading certain instances.
% % where the request scheduling is also highly relevant to the memory usage of the instances. 
% % the dynamic memory allocation approach would prefer a load-balancing policy to reduce preemptions of running requests on overloaded instances. 
% % Note that the load balancing can hardly be optimal as the growth of the sequences (and the load) is unknown at the scheduling time.
% However, when considering incoming requests, another objective is to reduce the queuing delays, especially for long input sequences that require large amounts of memory. Then the preferred choice might instead be packing requests to fewer instances to leave other instances free to accommodate long inputs. With
% unpredictable request arrivals and sequence lengths, it is difficult for the scheduling policy to navigate the tradeoff between the conflicting objectives.

We argue that the challenges above call for \emph{runtime rescheduling} of requests to react to the unpredictable memory demands and dynamic instance loads.
A simple intuition is that 
when the memory of an instance is insufficient (for running or new requests), it is possible that the whole cluster still has enough space; this is a natural consequence of the varying requests lengths and memory loads across instances.
Runtime rescheduling enables the system to harvest such free memory space throughout the cluster whenever needed.
% Unfortunately, existing systems cannot harvest such free memory space on other instances because requests are tied on the same instance throughout the execution once being scheduled.

We introduce \sysname{}, a new LLM serving system that exploits request rescheduling to maximize cluster memory utilization, thereby delivering high throughput and low latency. 
Such rescheduling is powered by efficient \emph{migration} of running requests along with their KV cache across instances. 

Straightforward rescheduling implementations would introduce substantial latency penalty to rescheduled requests, especially for long sequences.
% due to the overheads like recomputation. 
In comparison, \sysname{}'s migration mechanism is highly efficient in that it introduces \emph{near-zero} overhead that is \emph{constant} to the sequence length. This is achieved by carefully overlapping the computation and the KV cache transfer, leading to a negligible latency overhead even for very long sequences.

\sysname{} exploits request migration in three ways: (i) load-balance the instances to reduce request preemptions, improving performance isolation and tail latencies; (ii) make room for new requests with long input sequences, reducing the queuing delays (or the first-token latencies) and mitigating head-of-line blocking;
and (iii) quickly saturate new instances or drain out terminating instances, improving the efficiency of instance auto-scaling.
\sysname{} unifies these goals targeting different scenarios elegantly in one scheduling policy, leveraging the great scheduling flexibility enabled by request migration to react to specific situations.

% In summary, we make the following contributions: 

% 1. We identify the challenges in achieving efficient performance for long sequence LLM serving under latency SLO. 
% 2. We design and implement \sysname{}, an efficient and scalable distributed LLM serving platform powered by the KV cache migration mechanism and load-aware scheduling policy.
% 3. We evaluate \sysname{} on various scenarios and demonstrate that it substantially outperforms the previous state-of-the art solution vLLM.
